Align before Fuse: Vision and Language Representation Learning with Momentum Distillation

Large-scale vision and language representation learning has shown promising improvements on various vision-language tasks. Most existing methods employ a transformer-based multimodal encoder to jointly model visual tokens (region-based image features) and word tokens. Because the visual tokens and word tokens are unaligned, it is challenging for the multimodal encoder to learn image-text interactions. In this paper, we introduce a contrastive loss to ALign the image and text representations BEfore Fusing (ALBEF) them through cross-modal attention, which enables more grounded vision and language representation learning. Unlike most existing methods, our method does not require bounding box annotations nor high-resolution images. In order to improve learning from noisy web data, we propose momentum distillation, a self-training method which learns from pseudo-targets produced by a momentum model. We provide a theoretical analysis of ALBEF from a mutual information maximization perspective, showing that different training tasks can be interpreted as different ways to generate views for an image-text pair. ALBEF achieves state-of-the-art performance on multiple downstream vision-language tasks. On image-text retrieval, ALBEF outperforms methods that are pre-trained on orders of magnitude larger datasets. On VQA and NLVR$^2$, ALBEF achieves absolute improvements of 2.37% and 3.84% compared to the state-of-the-art, while enjoying faster inference speed. Code and pre-trained models are available at https://github.com/salesforce/ALBEF/.

==> table/nlvr.tex <==
\begin{table*}[!t]
    \aboverulesep = 0.55mm
    \belowrulesep = 0.55mm
	\small
	\centering	
	\setlength\tabcolsep{4pt}
	\resizebox{\textwidth}{!}{%
		\begin{tabular}	{l   |  c c  c  c c c c  |c  c }
			\toprule
			Method  & VisualBERT & LXMERT  & 12-in-1 & UNITER &  ViLT  & OSCAR & VILLA& Albef & Albef*\\
			\midrule
			dev  & 67.40  & 74.90 & -   & 77.14 & 75.24 & 78.07 & 78.39  & & \\
			test-P& 67.00& 74.50   & 78.87 & 77.87  & 76.21 & 78.36  & 79.30 & & \\		
			\bottomrule
		\end{tabular}
	}
	\caption
	{
		\small	
		NLVR$^2$
	}
	\label{tbl:nlvr}
\end{table*}	
